Knowledge Distillation via Token-level Relationship Graph

Knowledge distillation is a powerful technique for transferring knowledge from a pre-trained teacher model to a student model. However, the true potential of knowledge transfer has not been fully explored. Existing approaches primarily focus on distilling individual information or instance-level relationships, overlooking the valuable information embedded in token-level relationships, which may be particularly affected by the long-tail effects. To address the above limitations, we propose a novel method called Knowledge Distillation with Token-level Relationship Graph (TRG) that leverages the token-wise relational knowledge to enhance the performance of knowledge distillation. By employing TRG, the student model can effectively emulate higher-level semantic information from the teacher model, resulting in improved distillation results. To further enhance the learning process, we introduce a token-wise contextual loss called contextual loss, which encourages the student model to capture the inner-instance semantic contextual of the teacher model. We conduct experiments to evaluate the effectiveness of the proposed method against several state-of-the-art approaches. Empirical results demonstrate the superiority of TRG across various visual classification tasks, including those involving imbalanced data. Our method consistently outperforms the existing baselines, establishing a new state-of-the-art performance in the field of knowledge distillation.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> draft.tex <==
On the other hand, feature-based distillation involves aligning the intermediate features between the student and the teacher models to facilitate the distillation process. The loss function utilized in feature-based distillation takes the following form:
\begin{equation}
\label{Feature-based distill}
\mathcal{L}_{Fea}=\lambda_f\mathcal{L}_{F}\big(\Phi_{t}(F_{t}(x)), \Phi_{s}(F_{s}(x))\big) + \mathcal{L}_{logit},
\end{equation}
where $\Phi_{t}(f_{t}(x))$ and $\Phi_{s}(f_{s}(x))$ are denoted as transformation functions, they are typically employed when the feature maps of the teacher and student models do not have the same shape. The similarity function $\mathcal{L}_{F}(.)$ is utilized to align the feature maps of the teacher and student models.


In general, the distillation loss of relation-based knowledge based on the relations of feature maps can be formulated as
\begin{equation}
\label{RelD1}
L_{RelD}(f_{t}, f_{s})=\mathcal{L}_{R^{1}}\big(\Psi_{t}(\hat{f}_{t},\check{f}_{t}), \Psi_{s}(\hat{f}_{s},\check{f}_{s})\big)~,
\end{equation}
where $f_{t}$ and $f_{s}$ are the feature maps of teacher and student models, respectively. Pairs of feature maps are chosen from the teacher model, $\hat{f}_{t}$ and $\check{f}_{t}$, and from the student model, $\hat{f}_{s}$ and $\check{f}_{s}$. $\Psi_{t}(.)$ and $\Psi_{s}(.)$ are the similarity functions for pairs of feature maps from the teacher and student models. $\mathcal{L}_{R^{1}}(.)$ indicates the correlation function between the teacher and student feature maps.




information disparities 


where $\alpha$ represents the coefficient of Self-KD, and $\beta$ denotes the coefficient of residual loss for loss optimization. It is worth noting that due to the symmetry between the student model and pseudo-teacher model, the value of $\beta$ is doubled. The significance of the residual-based regularization is thoroughly discussed in Section~\ref{ablation}.


In ViT experiments, we follow the training pipeline proposed by Deit \cite{touvron2021training}, the only difference is that we add the graph distillation loss and contexture similarity loss to preserve inner-image and cross-image relational information during the distillation process:

However, in our case, the soft probability loss is applied specifically to the distillation token, as introduced in~\cite{touvron2021training}.

It is important to note that since we consider relationships across images, the tokens used to construct the token graph have the form of $B\cdot N\times D$, where $B$ denotes the batch size of the dataloader.

%Using the teacher's adjacency matrix as a mask, we can select the corresponding tokens from the student's representation to generate the student's token graph  using the k-NN distance defined by Eq.~\eqref{eq:knn}. 


\begin{table}[ht]
    \centering
    \caption{Top-1 accuracy (\%) comparison with Self-KD on TinyImageNet.}
    \begin{tblr}{
    hline{1,9} = {-}{0.08em},
    hline{2,8} = {-}{0.05em},
    }
        Method & WRB-16-2 & ResNet18 & DenseNet121 \\ 
        Baseline & 51.25\tiny{$\pm$0.20} & 55.70\tiny{$\pm$0.41} & 60.78\tiny{$\pm$0.27} \\ 
        DDGSD & 52.30\tiny{$\pm$0.27} & 57.76\tiny{$\pm$0.22} & 61.15\tiny{$\pm$0.23} \\ 
        BYOT & 51.43\tiny{$\pm$0.08} & 56.76\tiny{$\pm$0.41} & 61.61\tiny{$\pm$0.41} \\ 
        CS-KD & 52.23\tiny{$\pm$0.16} & 57.72\tiny{$\pm$0.10} & 62.04\tiny{$\pm$0.09} \\ 
        SLA+SD & 51.64\tiny{$\pm$0.35} & 58.67\tiny{$\pm$0.42} & 62.70\tiny{$\pm$0.21} \\ 
        BAKE & 53.12\tiny{$\pm$0.21} & 58.29\tiny{$\pm$0.34} & 62.20\tiny{$\pm$0.31} \\ 
        RSKD (ours) & \bf{53.42}\tiny{$\pm$\bf{0.28}} & \bf{59.20}\tiny{$\pm$\bf{0.38}} & \bf{63.60}\tiny{$\pm$\bf{0.32}} \\ 
    \end{tblr}
    \label{self-kd on tiny}
\end{table}

\begin{table}[ht]
    \centering
    \caption{Top-1 accuracy (\%) comparison with Self-KD on fine-grained datasets using ResNet18.}
    \scalebox{0.9}{
    \begin{tblr}{
    hline{1,9} = {-}{0.08em},
    hline{2,8} = {-}{0.05em},
    }
        Method & CUB200 & MIT67 & Dogs & Standford40 \\ 
        Baseline & 52.72\tiny{$\pm$1.34} & 56.07\tiny{$\pm$1.02} & 64.75\tiny{$\pm$0.20} & 44.30\tiny{$\pm$0.21} \\
        DDGSD & 58.79\tiny{$\pm$0.78} & 59.68\tiny{$\pm$0.86} & 69.20\tiny{$\pm$0.27} & 45.84\tiny{$\pm$1.72} \\
        BYOT & 58.86\tiny{$\pm$0.51} & 58.41\tiny{$\pm$0.71} & 68.92\tiny{$\pm$0.18} & 48.51\tiny{$\pm$1.02}\\
        CS-KD & 65.54\tiny{$\pm$0.10} & 61.18\tiny{$\pm$0.37} & 69.02\tiny{$\pm$0.40} & 47.34\tiny{$\pm$0.31}\\
        SLA+SD & 56.47\tiny{$\pm$0.81} & 61.59\tiny{$\pm$1.30} & 67.64\tiny{$\pm$0.34} & 54.67\tiny{$\pm$0.38}\\
        BAKE & \bf{70.26}\tiny{$\pm$\bf{0.25}} & 60.39\tiny{$\pm$0.55} & 70.26\tiny{$\pm$0.33} & 55.90\tiny{$\pm$0.21}\\ 
         (ours) & {68.97}\tiny{$\pm${0.31}} & {\bf {62.23}}\tiny{$\pm${\bf {0.55}}} & \bf{72.16}\tiny{$\pm${\bf {0.47}}} & {\bf {58.01}}\tiny{$\pm${\bf {0.61}}} \\
    \end{tblr}}
    \label{fine-grained results}
\end{table}


 For performance comparison, we run each experiment three times, and report the mean and standard deviation of the top-1 accuracy rate of the last epoch. The best results appear in {\bf bold}.
 \\

 {\noindent \bf Comparison with Self-Distillation Methods.} We present the results of our experiments on CIFAR-100 and TinyImageNet in Table~\ref{self-kd on cifar100} and Table~\ref{self-kd on tiny}, respectively. The \name method consistently outperforms other self-distillation baselines across different architecture settings. Notably, we observe that \name achieves a consistently higher top-1 accuracy rate than state-of-the-art approaches. On the CIFAR-100 dataset, our plain residual distillation approach improves the validation performance by an average of 0.6\%. Specifically, on ResNet18 network, our method increases the accuracy rate by 0.73\%, and on DenseNet121 network, it improves the accuracy rate by 1.44\%.Similarly, on TinyImageNet dataset, our proposed method enhances the test accuracy by 0.91\% using the ResNet18 architecture and by 0.90\% using the DenseNet121 architecture. These results provide compelling evidence for the effectiveness of our approach.

 In Table~\ref{fine-grained results}, we compare \name with other self-distillation methods on fine-grained datasets. In particular, our proposed approach improves the top-1 accuracy rate of the baselines from 56.07\% to 62.23\% on the MIT67 dataset, from 64.75\% to 72.16\% on the Stanford Dogs recognition fine-grained dataset. Also, on the Stanford40 Actions dataset, we enhance the accuracy from 44.30\% to 58.01\%. All these results demonstrate the effectiveness of leveraging residual learning to effectively utilize intermediate semantic features. This approach successfully mitigates the knowledge gap that exists between the output of the pseudo-teacher and the student model, as well as resolves the challenge of maintaining consistency between feature layers and output layers. Consequently, our proposed method holds great potential for application on lightweight devices, as it does not require additional computational resources. This highlights the practicality and efficiency of our approach in real-world scenarios.
\\

% \usepackage{tabularray}
\begin{table}
\centering
\caption{Top-1 accuracy (\%) comparison with other regularization methods on CIFAR-100.}
\label{regularization results}
\begin{tblr}{
  hline{1,6} = {-}{0.08em},
  hline{2,5} = {-}{0.05em},
}
Method        & ResNet18        & ResNet34 & DenseNet121    \\
Label-smoothing       & 77.31\tiny{$\pm{0.31}$}  & 78.01\tiny{$\pm{0.13}$}  & 77.77\tiny{$\pm{0.06}$} \\
Max-entropy           & 77.28\tiny{$\pm{0.35}$} & 77.90\tiny{$\pm{0.16}$} & 77.13\tiny{$\pm{0.43}$} \\
Spectral-Norm         & 76.18\tiny{$\pm{0.35}$}  & 76.90\tiny{$\pm{0.32}$}  & 77.09\tiny{$\pm{0.31}$} \\
RSKD (ours) &  
\bf{79.43}\tiny{$\pm{\bf 0.21}$}  & \bf{79.70}\tiny{$\pm{\bf0.26}$}  & 
\bf{79.83}\tiny{$\pm{\bf0.23}$} 
\end{tblr}
\end{table}


\begin{table}
\centering
\caption{Controlled experiments using the residual link removed model on CIFAR-100.}
\begin{tblr}{
  hline{1,4} = {-}{0.08em},
  hline{2,3} = {-}{0.05em},
}
Method & WRN-16-2 & ResNet18 & DenseNet121 \\
w/o Res.      &     72.14\tiny{$\pm$0.25}     &    77.92\tiny{$\pm$0.26}      &   78.01\tiny{$\pm$0.41}          \\
RSKD         &    \bf{74.20}\tiny{$\pm${\bf 0.31}}      &   \bf{79.43}\tiny{$\pm${\bf 0.21}}       &  \bf{79.83}\tiny{$\pm${\bf 0.23}}           
\end{tblr}
\label{compared results on cifar100}
\end{table}

\begin{table}
\centering
\caption{Controlled experiments using the residual link removed model on TinyImageNet.}
\begin{tblr}{
  hline{1,4} = {-}{0.08em},
  hline{2,3} = {-}{0.05em},
}
Method & WRN-16-2 & ResNet18 & DenseNet121 \\
w/o Res.      &     51.98\tiny{$\pm$0.31}     &   57.22\tiny{$\pm$0.27}      &   61.22\tiny{$\pm$0.25}          \\
RSKD         &    {\bf 53.42}\tiny{$\pm${\bf 0.28}}     &   {\bf 59.20}\tiny{$\pm${\bf 0.38}}      & {\bf 63.60}\tiny{$\pm${\bf 0.32}}          
\end{tblr}
\label{compared results on tinyimagenet}
\end{table}


To further validate the effectiveness of our proposed \name method, we conduct ablation studies to analyze various aspects of its performance. Specifically, we investigate the impact of the residual modules, different types of residual losses, the optimal choice of the residual coefficient hyperparameter, and the order of residual computation for the residual optimization. By conducting these ablation studies, we aim to gain deeper insights into the function and effectiveness of our method. The results and analysis of these studies are presented in the following sections, which shed light on the contributions and performance of each component in \name.\\ 




\begin{minipage}{\textwidth}
\begin{minipage}[h]{0.45\textwidth}
   \centering
    \includegraphics[scale=0.35]{body/pic/klmcd.pdf}
    \makeatletter\def\@captype{figure}\makeatother\caption{Graph}
\end{minipage}
\begin{minipage}[h]{0.45\textwidth}
\centering
\begin{tabular}{|c|c|} 
\hline 
aa & bb \\ 
\hline 
cc & dd \\ 
\hline 
\end{tabular} 
\makeatletter\def\@captype{table}\makeatother\caption{Table}  
\end{minipage}
\end{minipage}


\begin{minipage}{0.5\linewidth}
 \resizebox{\textwidth}{10mm}{
        \begin{tabular}{cccc}
   \toprule
   Temperature & Mean KLD($10^{-3}$) & MCD & Accuracy \\
   \midrule
   $0.02$ & $2.31$ &  $0.03$  & $75.99$\\
   $0.03$ & $2.22$  &  $0.04$  & $75.61$\\
   $0.05$ & $2.47$ & $0.06$ & $75.78$\\
   $Dynamic$ & $1.87$ & $0.07$ & $76.42$\\
   \bottomrule
\end{tabular}}
        \captionof{table}{The table illustrates the relationship between Mean KL Divergence, accuracy and Mean Cluster Distance over several fixed temperature and our dynamic temperature.}%这里必须写table，不然标题就自动设置成figure
        \label{tbl:dynamic}
	    \end{minipage}



     By considering both the instance-level and token-level graphs, our proposed approach provides a holistic understanding of the data, enabling a more robust knowledge transfer process. This comprehensive representation allows the student model to gain a deeper insight into the complex relationships and intricate details, leading to enhanced distillation performance and improved knowledge acquisition.


     In Fig.~\ref{fig:token-instance}, we compare the potential information embedded in instance-level graph and token-level graph. The token-level graph, in particular, takes into account the intricate details and patterns present in different patches of an image. For example, in an image with labels \textit{cat} and \textit{dog}, the fur patches of both animals should exhibit similar patterns.  Thus, we assume using token-level graph  to transfer knowledge may complements the instance-level knowledge, enabling a more comprehensive representation of the relationships and similarities among different elements across different images. This, in turn, contributes to the improved performance of the distillation process and enhances the student's ability to capture and replicate the knowledge present in the teacher model.


\subsection{Baselines}
We provide a concise overview of several knowledge distillation methods, including recent advancements in this field. Additionally, we highlight the significance of relational-based (including several graph-based) KD techniques as important baselines for comparison. 
\begin{itemize}
    \item {\bf KD}~\cite{hinton2015distilling} firstly introduces the idea of knowledge distillation by using soften logits of the teacher.
    \item {\bf FitNet}~\cite{romero2014fitnets} adds feature alignment to learn the rich information of intermediate features.
    \item {\bf AT}~\cite{zagoruyko2016paying} improves the knowledge distillation by forcing the student to learn the teacher's attention map.
    \item {\bf FT}~\cite{kim2018paraphrasing} introduces the so called “factors” as a more understandable form of intermediate representations.
    \item {\bf AB}~\cite{heo2019knowledge} proposes to use the activation boundary of the hidden neurons for knowledge transfer.
    \item {\bf SemCKD}~\cite{chen2021cross} introduces semantic calibration to automatically assigns proper target layers of the teacher model for each student layer with an attention mechanism.
    \item {\bf DIST}~\cite{huang2022knowledge} proposes a correlation-based loss to capture the intrinsic inter-class relations from the teacher explicitly.
    \item {\bf DKD}\cite{zhao2022decoupled} introduces a decoupled approach to soft logit distillation, dividing it into two distinct components: target classification knowledge distillation (TCKD) and non-target classification knowledge distillation (NCKD). This decoupling allows the student model to concentrate on the essential aspects of the knowledge being transferred.
\end{itemize}

To showcase the effectiveness of our approach in capturing relational knowledge, we do comparison with several existing relation-based (including several graph-based) KD methods listed below.
\begin{itemize}
    \item {\bf SP}~\cite{tung2019similarity} employs similarity-preserving knowledge to facilitate the training of a student network. This approach aims to ensure that input pairs, which elicit similar (or dissimilar) activations in the teacher network, yield corresponding similar (or dissimilar) activations in the student network.
    \item  {\bf CRD}~\cite{tian2019contrastive} introduces the contrastive loss to transfer pair-wise relationship across different networks.
    \item {\bf RKD}~\cite{park2019relational} proposes distance-wise and angle-wise distillation losses which aims to penalize structural differences in relations.
    \item {\bf CC}~\cite{peng2019correlation} proposes correlation congruence to transfer the knowledge of correlation between instances.
    \item {\bf IRG}~\cite{liu2019IRG} first proposes to use graph structure to represent the instance-wise relationship to distill the relational knowledge.
    \item {\bf HKD}~\cite{zhou2021distilling} proposes to distill the holistic knowledge based on an attributed graph constructed among instances.
\end{itemize}
